Signals of a Light Dark Force in the Galactic Center

Recent evidence for an excess of gamma rays in the GeV energy range about the Galactic Center have refocused attention on models of dark matter in the low mass regime ($m_\chi \lesssim m_Z/2$). Because this is an experimentally well-trod energy range, it can be a challenge to develop simple models that explain this excess, consistent with other experimental constraints. We reconsider models where the dark matter couples to dark photon, which has a weak kinetic mixing to the Standard Model photon, or scalars with a weak mixing with the Higgs boson. We focus on the light ($\lesssim 1.5 GeV$) dark mediator mass regime. Annihilations into the dark mediators can produce observable gamma rays through decays to $\pi^0$, through radiative processes when decaying to charged particles ($e^+e^-, \mu^+\mu^-,...$), and subsequent interactions of high energy $e^+e^-$ with gas and light. However, these models have no signals of $\bar p$ production, which is kinematically forbidden. We find that in these models, the shape of resulting gamma-ray spectrum can provide a good fit to the excess at Galactic Center. We discuss further constraints from AMS-02, and find regions of compatibility.

==> Cons.tex <==
\section{Constraints}
\label{sec:constraint}
Constraints on this scenario can be grouped into constraints on the signals of the DM, itself, or on the dark mediator.

\subsection{ Constraints on $\epsilon$}
The constraints on the mediator are strongest when it is a dark photon, and come
mainly related to its mixing parameter with Standard Model, $\epsilon$. These limits are
derived from searches in beam-dump experiments, fixed target experiments, and
e-e collisions, among others. For a given DM mass $m_\chi$ and
DM coupling to the dark photon, $g_X$, a constraint can also be derived from
DM direct detection searches. These constraints are summarized in
Figure ~\ref{fig:PS-darkphoton}.


\begin{figure*}
   \includegraphics[width=0.7\textwidth] {plots/A-visible-large-PS-101.pdf}
   \caption{ Parameter space for Dark Photon \label{fig:PS-darkphoton}.
Diagonal lines : contours of spin-independent direct detection constraints
for different DM mass from LUX and superCDMS.
Backgrounds shows current dark photon
constraints from other dark photon search~\cite{Essig:2013lka}.  These limits do not apply to the scalar mediator, or pseudo-Dirac DM case.}
\end{figure*}

Figure ~\ref{fig:PS-darkphoton} shows the parameter space for dark photon.
The beam dump experiments, such as E141~\cite{Riordan:1987aw},
E137~\cite{Bjorken:1988as}, E774~\cite{Bross:1989mp}, etc used the displaced
decay vertex covering the lower left corner of the parameter space.
The fixed target experiments, the anomalous magnetic moment measurement and
$e^+ e^-$ and hadronic collisions give the constraints on the upper part of the
space. Much of the high mass range has been explored by the BaBar experiment  \cite{Lees:2014xha}. There is much parameter space left for the dark photon search in the
dark photon mass from $10 ~\mev$ to a few $\gev$, although this is now being probed by MaMi \cite{Merkel:2011ze}, APEX \cite{Abrahamyan:2011gv}, HPS \cite{hpsweb}, and DarkLight \cite{Kahn:2013nma}, among others.

We display the constraints from direct detection on this plot as well. DM-nucleus scattering arises via dark photon exchange. The DM-proton scattering cross section is
\begin{equation}
   \sigma_p \simeq   \frac{\epsilon^2 ~ g_X^2 ~ e^2}{\pi}   \frac{\mu_{\chi p}^2 }{ m_{A'}^4}
            \simeq  1 \times 10^{-43} cm^2
         \left( \frac{ g_X}{0.1} \right)^2
         \left( \frac{ \epsilon}{1 \times 10^{-8}} \right)^2
         \left( \frac{ 0.1 \GeV}{ m_{A'} }\right)^4
\end{equation}
where $\mu_{\chi p}$ is the DM and proton reduced mass. 

This expression assumes the dark photon mass is larger than the t-channel momentum transfer of the scattering process. Considering $O(10)\gev$\, DM, the dark photon mass should be larger than $O(10)\mev$ for this assumption to be valid. For smaller dark photon mass, this breaks down and the t-channel momentum transfer becomes important. To clarify this effect we have inserted a momentum transfer of \nw{what amount} into the propagator \nw{for cdms and a different amount(?) for LUX}. This changes the behavior of the limits in Figure ~\ref{fig:PS-darkphoton}, and we have dashed the regions where this occurs, in which case this limits are only approximate. With DM mass given, we can fix $g_X$ through relic density, (e.g. for $m_\chi =10\gev$, $g_X = 0.06$). In Figure ~\ref{fig:PS-darkphoton},
superCDMS~\cite{Agnese:2014aze} and LUX~\cite{Akerib:2013tjd} are considered,
which are current best constraints of
spin-independent cross section at the DM mass range of 5~$\GeV$ - 30~$\GeV$.

Crucially, however, is that these limits are {\em only} present if the dark matter is a Dirac fermion. If the DM is split into a pseudo-Dirac state after U(1) breaking, then the scattering is inelastic and can be kinematically suppressed \cite{TuckerSmith:2001hy}, leaving no appreciable constraint on these models.

Additionally, these constraints are on the dark photon model. For the dark scalar, with its weaker interaction with ordinary matter, both the production and direct detection constraints are weaker.


















==> Makefile <==
# Makefile for LaTeX files

# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile

# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.

# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo

# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 

# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 

# $Id: Makefile,v 1.18 2006-06-19 10:58:11 mairas Exp $

LATEX	= latex
BIBTEX	= bibtex
MAKEINDEX = makeindex
XDVI	= xdvi -gamma 4
DVIPS	= dvips
DVIPDF  = dvipdft
L2H	= latex2html
GH	= gv

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

DATE=$(shell date +%Y-%m-%d)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false

# These are OK

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG	= $(SRC:%.tex=%.dvi)
PSF	= $(SRC:%.tex=%.ps)
PDF	= $(SRC:%.tex=%.pdf)

# These are not

#BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
#DEP     := $(shell perl -ne '($$_)=/^[^%]*\\include\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $(SRC))
#EPSPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $(SRC) $(DEP))


define run-latex
	$(COPY);$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

define run-pdflatex
	LATEX=pdflatex
	@$(run-latex)
endef

define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef

define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef

define geteps
	epses=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $< $$deps`
endef

define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef

all 	: $(TRG)

.PHONY	: all show clean ps pdf showps veryclean

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d)

veryclean	: clean
	  -rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.ps  *~

#$(geteps) ; echo $$epses ; \
# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	$(get_dependencies) ; echo $$deps ; \
	$(getbibs) ; echo $$bibs ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $$bibs $$epses $$mandeps" > $@ 

include $(SRC:.tex=.d)

# $(DEP) $(EPSPICS) $(BIBFILE)
$(TRG)	: %.dvi : %.tex
	  @$(run-latex)

$(PSF)	: %.ps : %.dvi
	  @$(DVIPS) $< -o $@

#$(PDF)  : %.pdf : %.dvi
	 # @$(DVIPDF) -o $@  $<
# To use pdflatex, comment the two lines above and uncomment the lines below
$(PDF) : %.pdf : %.tex
	@$(run-pdflatex)


show	: $(TRG)
	  @for i in $(TRG) ; do $(XDVI) $$i & done

showps	: $(PSF)
	  @for i in $(PSF) ; do $(GH) $$i & done

ps	: $(PSF) 

pdf	: $(PDF) 

# TODO: This probably needs fixing
html	: @$(DEP) $(EPSPICS)
	  @$(L2H) $(SRC)



######################################################################
# Define rules for EPS source files.

# These rules probably just cause unnecessary confusion, so commenting
# them away for the time being. -- mairas 2005-01-12

#%.eps: %.sxd
#	$(OUTDATED)
#%.eps: %.sda
#	$(OUTDATED)
#%.eps: %.png
#	$(OUTDATED)
#%.eps: %.sxc
#	$(OUTDATED)
#%.eps: %.xcf
#	$(OUTDATED)
#%.eps: %.zargo
#	$(OUTDATED)
#%.eps: %.m
#	@egrep -q $(MPRINT) $< && ($(OUTDATED))


==> spectrums.tex <==
\section{Photon Spectrum}

In this appendix, we will present the photon spectrum from different channels.

%\subsection{$\phi \rightarrow e^+ + e^-$}
\subsection{ FSR from $\phi \rightarrow f^+ + f^-$}
Final state radiation (FSR) gives the primary photon from the process of 
$\phi \rightarrow f^+ f^- $. At the rest frame of $\phi$, the photon energy 
spectrum is given by \cite{Birkedal:2005ep,
Mardon:2009rc},
\begin{equation}
 \frac{ \d N_\gamma} {\d x_0} = \frac{\alpha} {\pi} \frac{ 1+ ( 1-x_0)^2} {x_0} 
     \left[ -1 +  \ln \left( \frac{s ( 1-x_0)   } { m_f^2} \right) \right] \ ,
\end{equation} 
where $x_0 = 2 E_\gamma / \sqrt{s} =  2 E_\gamma / m_\phi$, and $m_f$ is the mass
of the fermion considering here. 
%Sustituting $m_e$ with its 
%mass, you will obtain the FSR of the charged fermion. 
To compute the photon spectrum from the one step cascade 
annihilation one should boost the $\phi$ field in the DM rest frame, 
and in the limit of $ \frac{2 m_\phi} { m_\chi} \rightarrow 0$, the spectrum is computed by the convolution,
\begin{equation} 
   \frac{\d N}{ \d x_1} = \int^1_{x_1}  \frac{\d x_0}{x_0} \frac{ \d N} 
         {\d x_0}  \ .
\end{equation} 
The approximation is good in the case we study where the correction is 
$  \sim \frac{ m_\phi^2} { m_\chi^2} \sim \mathcal{O} (10^{-2})$. 
In the DM frame, the photon spectrum from one $\phi$ is 
\begin{equation}  
   \frac{ \d N_\gamma} { \d x_1 }  = \frac{ \alpha} { \pi} \frac{1} {x_1} 
      \left[      
            \left( -1 + \ln \frac{ m_\phi^2} {m_f^2}  \right) R_1(x) + S_1(x)
      \right] \ ,
\end{equation}  
where 
\begin{eqnarray}
   R_1(x) &=& 2 -x  - x^2 + 2 x \ln x 
   \\ 
   S_1(x) &=& \left( \frac{\pi^2}{3 } - 1 \right) x + x^2 + 2x \ln x 
      + \left( 2- x- x^2 \right) \ln (1-x)  - 2 x \mathrm{Li}_2 (x) 
\end{eqnarray}

 
\subsection{ FSR from $\phi \rightarrow \pi^+ + \pi^-$}
The FSR in pion pair production is different from the fermion pair production 
due to the two facts: bosonic field and the form factor of the pion. The 
composite structure of the pion makes the computation of pion FSR have large 
theoretical uncertainties ~\cite{Gluza:2002ui}. Accepting the uncertainties,
scalar QED is one way to derive the FSR spectrum \cite{Gluza:2002ui}, in which
the spectrum is divided into hard photon spectrum and soft-virtual one,
\begin{equation}
   \frac{\d N_\gamma } { d x_1} =   \frac{\alpha}{\pi} 
      \left[
      \delta^{V+S}  + x^{ B_\pi (x) -1} B_\pi ( s, x)  + \delta^H ( x)
      \right]
\end{equation}
where
\begin{eqnarray}
   \delta^H ( x) &=&  2 x \frac{\beta_\pi^\prime } 
         { \beta_\pi^3  }
\\
   B_\pi (x) &=& \frac{ 2 ( 1-x) \beta_\pi^\prime} { \beta_\pi}
      \left[ 
      \frac{ 1+ {\beta_\pi^\prime}^2 }{ 2 \beta_\pi}
      \ln \left( \frac{1 + \beta_\pi^\prime} { 1- \beta_\pi^\prime} \right) -1 
      \right]
\\
   \delta^{V+S}  &=& \frac{  2 + \beta_\pi^2}{ \beta_\pi} 
      \ln \left( \frac{ 1+ \beta_\pi} {1- \beta_\pi} \right)  -2 
      - 2 \ln \left( \frac{ 1 - \beta_\pi^2 }{4} \right)
      -\frac{  1+ \beta_\pi^2}{ 2\beta_\pi}  
      \left\{ 
         \ln \left( \frac{ 1+ \beta_\pi }{ 1- \beta_\pi}\right)
         \left[ 
            \ln \left( \frac{ 1+ \beta_\pi }{2} \right)
            + \ln \beta_\pi
         \right] + \right.
\nonumber\\
      &&
      \left.
       \ln \left( \frac{ 1+ \beta_\pi }{ 2 \beta_\pi}\right)
       \ln \left( \frac{ 1- \beta_\pi }{ 2 \beta_\pi}\right)
         + 2 \mathrm{Li}_2 \left( \frac{ 2 \beta_\pi }{ 1+ \beta_\pi}\right)
         + 2 \mathrm{Li}_2 \left( -\frac{ 1- \beta_\pi }{ 2 \beta_\pi}\right)
         -\frac{ 2 }{3} \pi^2
      \right\}
\end{eqnarray}
and $\beta_pi$ is the pion velocity $ \beta_\pi  = \sqrt{ 1 - 4 m_\pi^2 /s }$,
$ \beta_\pi^\prime  = \sqrt{ 1 - 4 m_\pi^2 /((1-x)s ) }$. After the production
of the pion, the cascade decay of $\pi$ to $\mu$ will also contribute to the 
photon spectrum.
   























